The Modular Audio Recognition Framework (MARF) and its Applications: Scientific and Software Engineering Notes

MARF is an open-source research platform and a collection of voice/sound/speech/text and natural language processing (NLP) algorithms written in Java and arranged into a modular and extensible framework facilitating addition of new algorithms. MARF can run distributively over the network and may act as a library in applications or be used as a source for learning and extension. A few example applications are provided to show how to use the framework. There is an API reference in the Javadoc format as well as this set of accompanying notes with the detailed description of the architectural design, algorithms, and applications. MARF and its applications are released under a BSD-style license and is hosted at SourceForge.net. This document provides the details and the insight on the internals of MARF and some of the mentioned applications.

==> old-results.tex <==
\begin{verbatim}
1st & -boost -fft -eucl &  20 & 13 & 60.60606060606061
2nd & -boost -fft -eucl &  25 & 8 & 75.75757575757575
1st & -low -lpc -eucl &  18 & 15 & 54.54545454545454
2nd & -low -lpc -eucl &  21 & 12 & 63.63636363636363
1st & -norm -fft -cheb &  26 & 7 & 78.78787878787878
2nd & -norm -fft -cheb &  28 & 5 & 84.84848484848484
1st & -boost -lpc -eucl &  24 & 10 & 70.58823529411765
2nd & -boost -lpc -eucl &  28 & 6 & 82.35294117647058
1st & -norm -lpc -cheb &  23 & 10 & 69.6969696969697
2nd & -norm -lpc -cheb &  26 & 7 & 78.78787878787878
1st & -high -fft -eucl &  23 & 10 & 69.6969696969697
2nd & -high -fft -eucl &  29 & 4 & 87.87878787878788
1st & -high -lpc -cheb &  21 & 12 & 63.63636363636363
2nd & -high -lpc -cheb &  24 & 9 & 72.72727272727273
1st & -low -fft -eucl &  22 & 11 & 66.66666666666666
2nd & -low -fft -eucl &  27 & 6 & 81.81818181818183
1st & -norm -fft -eucl &  22 & 11 & 66.66666666666666
2nd & -norm -fft -eucl &  29 & 4 & 87.87878787878788
1st & -boost -fft -cheb &  23 & 11 & 67.64705882352942
2nd & -boost -fft -cheb &  25 & 9 & 73.52941176470588
1st & -norm -lpc -eucl &  23 & 10 & 69.6969696969697
2nd & -norm -lpc -eucl &  26 & 7 & 78.78787878787878
1st & -low -lpc -cheb &  20 & 13 & 60.60606060606061
2nd & -low -lpc -cheb &  23 & 10 & 69.6969696969697
1st & -boost -lpc -cheb &  23 & 10 & 69.6969696969697
2nd & -boost -lpc -cheb &  27 & 6 & 81.81818181818183
1st & -high -fft -cheb &  22 & 11 & 66.66666666666666
2nd & -high -fft -cheb &  29 & 4 & 87.87878787878788
1st & -high -lpc -eucl &  20 & 13 & 60.60606060606061
2nd & -high -lpc -eucl &  23 & 10 & 69.6969696969697
1st & -low -fft -cheb &  20 & 13 & 60.60606060606061
2nd & -low -fft -cheb &  22 & 11 & 66.66666666666666



\begin{verbatim}
& -boost -fft -eucl &  9 & 4 & 69.23076923076923
& -boost -fft -cheb &  9 & 4 & 69.23076923076923

& -boost -lpc -eucl &  8 & 5 & 61.53846153846154
& -boost -lpc -cheb &  9 & 4 & 69.23076923076923

& -fft -cheb &  11 & 2 & 84.61538461538461
& -fft -eucl &  10 & 3 & 76.92307692307693

& -lpc -cheb &  9 & 4 & 69.23076923076923
& -lpc -eucl &  9 & 4 & 69.23076923076923

with 2nd guess:
1st & -boost -fft -eucl &  12 & 6 & 66.66666666666666
2nd & -boost -fft -eucl &  15 & 3 & 83.33333333333334
1st & -fft -cheb &  14 & 4 & 77.77777777777779
2nd & -fft -cheb &  15 & 3 & 83.33333333333334
1st & -boost -lpc -cheb &  11 & 7 & 61.111111111111114
2nd & -boost -lpc -cheb &  13 & 5 & 72.22222222222221
1st & -fft -eucl &  12 & 6 & 66.66666666666666
2nd & -fft -eucl &  16 & 2 & 88.88888888888889
1st & -lpc -cheb &  12 & 6 & 66.66666666666666
2nd & -lpc -cheb &  14 & 4 & 77.77777777777779
1st & -boost -lpc -eucl &  10 & 8 & 55.55555555555556
2nd & -boost -lpc -eucl &  12 & 6 & 66.66666666666666
1st & -boost -fft -cheb &  11 & 7 & 61.111111111111114
2nd & -boost -fft -cheb &  12 & 6 & 66.66666666666666
1st & -lpc -eucl &  12 & 6 & 66.66666666666666
2nd & -lpc -eucl &  14 & 4 & 77.77777777777779


~1000 Hz, 15
1st & -boost -fft -eucl &  11 & 7 & 61.111111111111114
2nd & -boost -fft -eucl &  14 & 4 & 77.77777777777779
1st & -fft -cheb &  14 & 4 & 77.77777777777779
2nd & -fft -cheb &  15 & 3 & 83.33333333333334
1st & -boost -lpc -cheb &  12 & 6 & 66.66666666666666
2nd & -boost -lpc -cheb &  14 & 4 & 77.77777777777779
1st & -fft -eucl &  12 & 6 & 66.66666666666666
2nd & -fft -eucl &  16 & 2 & 88.88888888888889
1st & -lpc -cheb &  12 & 6 & 66.66666666666666
2nd & -lpc -cheb &  14 & 4 & 77.77777777777779
1st & -boost -lpc -eucl &  12 & 6 & 66.66666666666666
2nd & -boost -lpc -eucl &  14 & 4 & 77.77777777777779
1st & -boost -fft -cheb &  12 & 6 & 66.66666666666666
2nd & -boost -fft -cheb &  13 & 5 & 72.22222222222221
1st & -lpc -eucl &  12 & 6 & 66.66666666666666
2nd & -lpc -eucl &  14 & 4 & 77.77777777777779



1st & -boost -fft -eucl &  11 & 7 & 61.111111111111114
2nd & -boost -fft -eucl &  14 & 4 & 77.77777777777779
1st & -low -lpc -eucl &  10 & 8 & 55.55555555555556
2nd & -low -lpc -eucl &  12 & 6 & 66.66666666666666
1st & -norm -fft -cheb &  14 & 4 & 77.77777777777779
2nd & -norm -fft -cheb &  15 & 3 & 83.33333333333334
1st & -boost -lpc -eucl &  12 & 6 & 66.66666666666666
2nd & -boost -lpc -eucl &  14 & 4 & 77.77777777777779
1st & -norm -lpc -cheb &  12 & 6 & 66.66666666666666
2nd & -norm -lpc -cheb &  14 & 4 & 77.77777777777779
1st & -high -fft -eucl &  12 & 6 & 66.66666666666666
2nd & -high -fft -eucl &  16 & 2 & 88.88888888888889
1st & -high -lpc -cheb &  11 & 7 & 61.111111111111114
2nd & -high -lpc -cheb &  13 & 5 & 72.22222222222221
1st & -low -fft -eucl &  12 & 6 & 66.66666666666666
2nd & -low -fft -eucl &  15 & 3 & 83.33333333333334
1st & -norm -fft -eucl &  12 & 6 & 66.66666666666666
2nd & -norm -fft -eucl &  16 & 2 & 88.88888888888889
1st & -boost -fft -cheb &  12 & 6 & 66.66666666666666
2nd & -boost -fft -cheb &  13 & 5 & 72.22222222222221
1st & -norm -lpc -eucl &  12 & 6 & 66.66666666666666
2nd & -norm -lpc -eucl &  14 & 4 & 77.77777777777779
1st & -low -lpc -cheb &  11 & 7 & 61.111111111111114
2nd & -low -lpc -cheb &  13 & 5 & 72.22222222222221
1st & -boost -lpc -cheb &  12 & 6 & 66.66666666666666
2nd & -boost -lpc -cheb &  14 & 4 & 77.77777777777779
1st & -high -fft -cheb &  12 & 6 & 66.66666666666666
2nd & -high -fft -cheb &  16 & 2 & 88.88888888888889
1st & -high -lpc -eucl &  10 & 8 & 55.55555555555556
2nd & -high -lpc -eucl &  13 & 5 & 72.22222222222221
1st & -low -fft -cheb &  11 & 7 & 61.111111111111114
2nd & -low -fft -cheb &  12 & 6 & 66.66666666666666


only one sample in testing set

1st & -boost -fft -eucl &  20 & 13 & 60.60606060606061
2nd & -boost -fft -eucl &  25 & 8 & 75.75757575757575
1st & -low -lpc -eucl &  18 & 15 & 54.54545454545454
2nd & -low -lpc -eucl &  21 & 12 & 63.63636363636363
1st & -norm -fft -cheb &  26 & 7 & 78.78787878787878
2nd & -norm -fft -cheb &  28 & 5 & 84.84848484848484
1st & -boost -lpc -eucl &  24 & 10 & 70.58823529411765
2nd & -boost -lpc -eucl &  28 & 6 & 82.35294117647058
1st & -norm -lpc -cheb &  23 & 10 & 69.6969696969697
2nd & -norm -lpc -cheb &  26 & 7 & 78.78787878787878
1st & -high -fft -eucl &  23 & 10 & 69.6969696969697
2nd & -high -fft -eucl &  29 & 4 & 87.87878787878788
1st & -high -lpc -cheb &  21 & 12 & 63.63636363636363
2nd & -high -lpc -cheb &  24 & 9 & 72.72727272727273
1st & -low -fft -eucl &  22 & 11 & 66.66666666666666
2nd & -low -fft -eucl &  27 & 6 & 81.81818181818183
1st & -norm -fft -eucl &  22 & 11 & 66.66666666666666
2nd & -norm -fft -eucl &  29 & 4 & 87.87878787878788
1st & -boost -fft -cheb &  23 & 11 & 67.64705882352942
2nd & -boost -fft -cheb &  25 & 9 & 73.52941176470588
1st & -norm -lpc -eucl &  23 & 10 & 69.6969696969697
2nd & -norm -lpc -eucl &  26 & 7 & 78.78787878787878
1st & -low -lpc -cheb &  20 & 13 & 60.60606060606061
2nd & -low -lpc -cheb &  23 & 10 & 69.6969696969697
1st & -boost -lpc -cheb &  23 & 10 & 69.6969696969697
2nd & -boost -lpc -cheb &  27 & 6 & 81.81818181818183
1st & -high -fft -cheb &  22 & 11 & 66.66666666666666
2nd & -high -fft -cheb &  29 & 4 & 87.87878787878788
1st & -high -lpc -eucl &  20 & 13 & 60.60606060606061
2nd & -high -lpc -eucl &  23 & 10 & 69.6969696969697
1st & -low -fft -cheb &  20 & 13 & 60.60606060606061
2nd & -low -fft -cheb &  22 & 11 & 66.66666666666666


1st & -norm -fft -eucl &  14 & 6 & 70.0
2nd & -norm -fft -eucl &  18 & 2 & 90.0
1st & -high -lpc -cheb &  12 & 8 & 60.0
2nd & -high -lpc -cheb &  14 & 6 & 70.0
1st & -low -fft -eucl &  14 & 6 & 70.0
2nd & -low -fft -eucl &  17 & 3 & 85.0
1st & -boost -fft -cheb &  14 & 6 & 70.0
2nd & -boost -fft -cheb &  15 & 5 & 75.0
1st & -norm -lpc -cheb &  13 & 7 & 65.0
2nd & -norm -lpc -cheb &  15 & 5 & 75.0
1st & -high -fft -eucl &  14 & 6 & 70.0
2nd & -high -fft -eucl &  18 & 2 & 90.0
1st & -low -lpc -eucl &  11 & 9 & 55.00000000000001
2nd & -low -lpc -eucl &  13 & 7 & 65.0
1st & -boost -lpc -cheb &  13 & 7 & 65.0
2nd & -boost -lpc -cheb &  15 & 5 & 75.0
1st & -high -lpc -eucl &  11 & 9 & 55.00000000000001
2nd & -high -lpc -eucl &  14 & 6 & 70.0
1st & -norm -fft -cheb &  16 & 4 & 80.0
2nd & -norm -fft -cheb &  17 & 3 & 85.0
1st & -boost -fft -eucl &  13 & 7 & 65.0
2nd & -boost -fft -eucl &  16 & 4 & 80.0
1st & -low -fft -cheb &  12 & 8 & 60.0
2nd & -low -fft -cheb &  14 & 6 & 70.0
1st & -norm -lpc -eucl &  13 & 7 & 65.0
2nd & -norm -lpc -eucl &  15 & 5 & 75.0
1st & -high -fft -cheb &  14 & 6 & 70.0
2nd & -high -fft -cheb &  18 & 2 & 90.0
1st & -boost -lpc -eucl &  13 & 7 & 65.0
2nd & -boost -lpc -eucl &  15 & 5 & 75.0
1st & -low -lpc -cheb &  13 & 7 & 65.0
2nd & -low -lpc -cheb &  15 & 5 & 75.0

Looks like our bests results are with -norm -fft -eucl , -high -fft -eucl
and -high -fft -cheb.

\end{verbatim}


==> output.tex <==
\tiny
\begin{verbatim}
Training...
Done training on folder "training-samples".
Done training on folder "training-samples".
Done training on folder "training-samples".
Done training on folder "training-samples".
Done training on folder "training-samples".
Done training on folder "training-samples".
Done training on folder "training-samples".
Done training on folder "training-samples".
Testing...
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 6
     Second Best Name: Margarita Mokhova
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 6
     Second Best Name: Margarita Mokhova
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 6
     Second Best Name: Margarita Mokhova
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 6
     Second Best Name: Margarita Mokhova
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/aihua5.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 14
     Expected Speaker: Aihua
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham13.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/graham14.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 9
     Expected Speaker: Graham
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ian15.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 2
     Expected Speaker: Ian
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/ira4.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 13
     Expected Speaker: Ira
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 6
     Second Best Name: Margarita Mokhova
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jihed3.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 10
     Expected Speaker: Jihed Halimi
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/jim6.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 4
     Expected Speaker: Jimmy
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/madhumita4.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 11
     Expected Speaker: Madhumita
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/michelle1.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 16
     Expected Speaker: Michelle
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 2
   Speaker identified: Ian
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/nick1.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 15
     Expected Speaker: Nick
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 18
     Second Best Name: Van Halen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 18
     Second Best Name: Van Halen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 18
     Second Best Name: Van Halen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 18
     Second Best Name: Van Halen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 19
   Speaker identified: RHCP
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 18
     Second Best Name: Van Halen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rhcp9.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 19
     Expected Speaker: RHCP
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/rita6.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 6
   Speaker identified: Margarita Mokhova
Expected Speaker's ID: 6
     Expected Speaker: Margarita Mokhova
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 7
     Second Best Name: Alexei Mokhov
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 7
   Speaker identified: Alexei Mokhov
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 7
   Speaker identified: Alexei Mokhov
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 16
   Speaker identified: Michelle
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 13
     Second Best Name: Ira
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/sei-sphere.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 7
     Expected Speaker: Alexei Mokhov
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 4
   Speaker identified: Jimmy
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/serge-label.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 1
     Expected Speaker: Serge
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 14
     Second Best Name: Aihua
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 10
   Speaker identified: Jihed Halimi
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/shabana8.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 17
     Expected Speaker: Shabana
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 14
   Speaker identified: Aihua
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test1.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 5
     Second Best Name: Dr. Suen
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve-test2.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 13
   Speaker identified: Ira
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 11
     Second Best Name: Madhumita
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 11
   Speaker identified: Madhumita
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 15
   Speaker identified: Nick
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 9
   Speaker identified: Graham
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 17
   Speaker identified: Shabana
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/steve2.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 3
   Speaker identified: Steve
Expected Speaker's ID: 3
     Expected Speaker: Steve
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 1
   Speaker identified: Serge
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 0
     Second Best Name: Unknown
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 1
     Second Best Name: Serge
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/suen2.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 5
   Speaker identified: Dr. Suen
Expected Speaker's ID: 5
     Expected Speaker: Dr. Suen
       Second Best ID: 3
     Second Best Name: Steve
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -norm -fft -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -norm -fft -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -norm -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 4
     Second Best Name: Jimmy
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -norm -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 9
     Second Best Name: Graham
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -boost -fft -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -boost -fft -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -boost -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -boost -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -low -fft -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -low -fft -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 15
     Second Best Name: Nick
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -low -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -low -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -high -fft -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -high -fft -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 2
     Second Best Name: Ian
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -high -lpc -eucl
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=-=
DOING FILE:
testing-samples/vanh9.wav
=============================================
               Config: -high -lpc -cheb
         Speaker's ID: 18
   Speaker identified: Van Halen
Expected Speaker's ID: 18
     Expected Speaker: Van Halen
       Second Best ID: 10
     Second Best Name: Jihed Halimi
---------------------------------------------
Stats:
1st CONFIG: -boost -fft -eucl , GOOD: 13, BAD: 7, %: 65.0
2nd CONFIG: -boost -fft -eucl , GOOD: 16, BAD: 4, %: 80.0
1st CONFIG: -low -lpc -eucl , GOOD: 11, BAD: 9, %: 55.00000000000001
2nd CONFIG: -low -lpc -eucl , GOOD: 13, BAD: 7, %: 65.0
1st CONFIG: -norm -fft -cheb , GOOD: 16, BAD: 4, %: 80.0
2nd CONFIG: -norm -fft -cheb , GOOD: 17, BAD: 3, %: 85.0
1st CONFIG: -boost -lpc -eucl , GOOD: 13, BAD: 7, %: 65.0
2nd CONFIG: -boost -lpc -eucl , GOOD: 15, BAD: 5, %: 75.0
1st CONFIG: -norm -lpc -cheb , GOOD: 13, BAD: 7, %: 65.0
2nd CONFIG: -norm -lpc -cheb , GOOD: 15, BAD: 5, %: 75.0
1st CONFIG: -high -fft -eucl , GOOD: 14, BAD: 6, %: 70.0
2nd CONFIG: -high -fft -eucl , GOOD: 18, BAD: 2, %: 90.0
1st CONFIG: -high -lpc -cheb , GOOD: 12, BAD: 8, %: 60.0
2nd CONFIG: -high -lpc -cheb , GOOD: 14, BAD: 6, %: 70.0
1st CONFIG: -low -fft -eucl , GOOD: 14, BAD: 6, %: 70.0
2nd CONFIG: -low -fft -eucl , GOOD: 17, BAD: 3, %: 85.0
1st CONFIG: -norm -fft -eucl , GOOD: 14, BAD: 6, %: 70.0
2nd CONFIG: -norm -fft -eucl , GOOD: 18, BAD: 2, %: 90.0
1st CONFIG: -boost -fft -cheb , GOOD: 14, BAD: 6, %: 70.0
2nd CONFIG: -boost -fft -cheb , GOOD: 15, BAD: 5, %: 75.0
1st CONFIG: -norm -lpc -eucl , GOOD: 13, BAD: 7, %: 65.0
2nd CONFIG: -norm -lpc -eucl , GOOD: 15, BAD: 5, %: 75.0
1st CONFIG: -low -lpc -cheb , GOOD: 13, BAD: 7, %: 65.0
2nd CONFIG: -low -lpc -cheb , GOOD: 15, BAD: 5, %: 75.0
1st CONFIG: -boost -lpc -cheb , GOOD: 13, BAD: 7, %: 65.0
2nd CONFIG: -boost -lpc -cheb , GOOD: 15, BAD: 5, %: 75.0
1st CONFIG: -high -fft -cheb , GOOD: 14, BAD: 6, %: 70.0
2nd CONFIG: -high -fft -cheb , GOOD: 18, BAD: 2, %: 90.0
1st CONFIG: -high -lpc -eucl , GOOD: 11, BAD: 9, %: 55.00000000000001
2nd CONFIG: -high -lpc -eucl , GOOD: 14, BAD: 6, %: 70.0
1st CONFIG: -low -fft -cheb , GOOD: 12, BAD: 8, %: 60.0
2nd CONFIG: -low -fft -cheb , GOOD: 14, BAD: 6, %: 70.0
Testing Done
\end{verbatim}


==> pparsing-sample-run.tex <==
\begin{verbatim}
junebug.mokhov [a3] % java ProbabilisticParsingApp --parse

Probabilistic Parsing
Serguei A. Mokhov, mokhov@cs
April 2003



Entering interactive mode... Type \q to exit.
sentence> my rabbit has a white smile
my rabbit has a white smile

Parse for the sentence [ my rabbit has a white smile ] is below:

SYNOPSIS:

<NONTERMINAL> (PROBABILITY) [ SPAN: words of span ]

<S> (0.0020480000000000008) [ 0-5: my rabbit has a white smile ]
        <NP> (0.04000000000000001) [ 0-1: my rabbit ]
                <DET> (0.1) [ 0-0: my ]
                <NOMINAL> (0.4) [ 1-1: rabbit ]
        <VP> (0.06400000000000002) [ 2-5: has a white smile ]
                <V> (0.8) [ 2-2: has ]
                <NP> (0.08000000000000002) [ 3-5: a white smile ]
                        <DET> (0.4) [ 3-3: a ]
                        <NOMINAL> (0.2) [ 4-5: white smile ]
                                <ADJ> (1.0) [ 4-4: white ]
                                <NOMINAL> (0.2) [ 5-5: smile ]


sentence> my rabbit has a smile
my rabbit has a smile

Parse for the sentence [ my rabbit has a smile ] is below:

SYNOPSIS:

<NONTERMINAL> (PROBABILITY) [ SPAN: words of span ]

<S> (0.0020480000000000008) [ 0-4: my rabbit has a smile ]
        <NP> (0.04000000000000001) [ 0-1: my rabbit ]
                <DET> (0.1) [ 0-0: my ]
                <NOMINAL> (0.4) [ 1-1: rabbit ]
        <VP> (0.06400000000000002) [ 2-4: has a smile ]
                <V> (0.8) [ 2-2: has ]
                <NP> (0.08000000000000002) [ 3-4: a smile ]
                        <DET> (0.4) [ 3-3: a ]
                        <NOMINAL> (0.2) [ 4-4: smile ]


sentence> my rabbit has a telephone
my rabbit has a telephone

There's no parse for [ my rabbit has a telephone ]

sentence> the cat eats the rabbit
the cat eats the rabbit

Parse for the sentence [ the cat eats the rabbit ] is below:

SYNOPSIS:

<NONTERMINAL> (PROBABILITY) [ SPAN: words of span ]

<S> (0.006400000000000002) [ 0-4: the cat eats the rabbit ]
        <NP> (0.2) [ 0-1: the cat ]
                <DET> (0.5) [ 0-0: the ]
                <NOMINAL> (0.4) [ 1-1: cat ]
        <VP> (0.04000000000000001) [ 2-4: eats the rabbit ]
                <V> (0.2) [ 2-2: eats ]
                <NP> (0.2) [ 3-4: the rabbit ]
                        <DET> (0.5) [ 3-3: the ]
                        <NOMINAL> (0.4) [ 4-4: rabbit ]


sentence> a white cat has a white smile
a white cat has a white smile

Parse for the sentence [ a white cat has a white smile ] is below:

SYNOPSIS:

<NONTERMINAL> (PROBABILITY) [ SPAN: words of span ]

<S> (0.008192000000000003) [ 0-6: a white cat has a white smile ]
        <NP> (0.16000000000000003) [ 0-2: a white cat ]
                <DET> (0.4) [ 0-0: a ]
                <NOMINAL> (0.4) [ 1-2: white cat ]
                        <ADJ> (1.0) [ 1-1: white ]
                        <NOMINAL> (0.4) [ 2-2: cat ]
        <VP> (0.06400000000000002) [ 3-6: has a white smile ]
                <V> (0.8) [ 3-3: has ]
                <NP> (0.08000000000000002) [ 4-6: a white smile ]
                        <DET> (0.4) [ 4-4: a ]
                        <NOMINAL> (0.2) [ 5-6: white smile ]
                                <ADJ> (1.0) [ 5-5: white ]
                                <NOMINAL> (0.2) [ 6-6: smile ]


sentence> cat white my has rabbit
cat white my has rabbit

There's no parse for [ cat white my has rabbit ]

sentence> smile rabbit eats my cat
smile rabbit eats my cat

There's no parse for [ smile rabbit eats my cat ]

sentence> cat eats rabbit
cat eats rabbit

There's no parse for [ cat eats rabbit ]

sentence> the cat eats the rabbit
the cat eats the rabbit

Parse for the sentence [ the cat eats the rabbit ] is below:

SYNOPSIS:

<NONTERMINAL> (PROBABILITY) [ SPAN: words of span ]

<S> (0.006400000000000002) [ 0-4: the cat eats the rabbit ]
        <NP> (0.2) [ 0-1: the cat ]
                <DET> (0.5) [ 0-0: the ]
                <NOMINAL> (0.4) [ 1-1: cat ]
        <VP> (0.04000000000000001) [ 2-4: eats the rabbit ]
                <V> (0.2) [ 2-2: eats ]
                <NP> (0.2) [ 3-4: the rabbit ]
                        <DET> (0.5) [ 3-3: the ]
                        <NOMINAL> (0.4) [ 4-4: rabbit ]


sentence> \q
junebug.mokhov [a3] %
\end{verbatim}


==> regression-app-usage.tex <==
\begin{verbatim}
Usage:
    java Regression --help | -h
        : to display this help and exit

    java Regression --version
        : to display version and exit

    java Regression [ --debug ] [ OPTIONS ]
        : to run the regression tests

Where options are of the following:

    --debug  - enable debugging (more verbose output)


\end{verbatim}


==> test-plugin-usage.tex <==
\begin{verbatim}

Usage:

    java TestPlugin [ LOADER ] [ PREP ] [ FEAT ] [ OPTIONS ]

       or

    java -jar TestPlugin.jar [ LOADER ] [ PREP ] [ FEAT ] [ OPTIONS ]

Where LOADER options one of the following:

    --uwav         unrestricted WAV loader (the default plugin)
    --sine         sine-wave 'loader'

Where PREPprocessing options one of the following:

    --random       random preprocessing (the default plugin)
    --raw          no preprocessing

Where FEATure extraction options one of the following:

    --hashadd      the hash-add plugin as feature extraction (default)
    --minmax       use min-max amplitudes as feature extraction
    --fft          use FFT as feature extraction
    --lpc          use LPC as feature extraction

Where options are one of the following:

    --wavegraph    dump CSV-formatted wave-graph values
    --help | -h    displays this help and exits
    --version      displays application and MARF versions
    --debug        run tests with the debug mode enabled

\end{verbatim}

